Evidence-based Factual Error Correction

This paper introduces the task of factual error correction: performing edits to a claim so that the generated rewrite is better supported by evidence. This extends the well-studied task of fact verification by providing a mechanism to correct written texts that are refuted or only partially supported by evidence. We demonstrate that it is feasible to train factual error correction systems from existing fact checking datasets which only contain labeled claims accompanied by evidence, but not the correction. We achieve this by employing a two-stage distant supervision approach that incorporates evidence into masked claims when generating corrections. Our approach, based on the T5 transformer and using retrieved evidence, achieved better results than existing work which used a pointer copy network and gold evidence, producing accurate factual error corrections for 5x more instances in human evaluation and a .125 increase in SARI score. The evaluation is conducted on a dataset of 65,000 instances based on a recent fact verification shared task and we release it to enable further work on the task.

==> 7_results.tex <==
\section{Implementation}
Schuster baseline: adapting code released in their public system. Masker + corrector, we consider the system as a whole, and also evaluate using their masker in context.
New masker-correctors. For the maskers, we use LIME on pre-trained FEVER system. We train the system with BERT classifier on the FEVER dataset following the training procedure from \citet{Thorne2018a}. The LIME explanations are generated with 250 samples with num\_features set to 6. The seq2seq corrector was built using a pre-trained T5 model \citep{Raffel2020}, fine tuned for 8 epochs with early stopping, minimizing the validation loss with the reference corrections.  The Language-model based masker and corrector were a BERT-base model. For surprisal, we break an $n$ word sentence in to $n$ masked word prediction tasks. We mask the top $k$ tokens ordered by loss.

\section{Initial Findings}
We first perform an experiment without information retrieval, just considering the error correction component, assuming perfect IR. This will allow us to know which metrics to optimize for when constructing the full system which incorporates a retriever.
The self-supervised Masker+Corrector (M+C) systems, baseline from \citet{Shah2019} and the fully-supervised baseline system are trained using the FEVER data discussed in Section~\ref{sec:data}.
Factual error corrections are made to the claims from the development split of the dataset and the generated outputs were collected. 

%{\color{red} TODO: finish reporting findings. Tables are finished, just needs more text}
The averaged scores from the manual evaluation are listed in Table~\ref{tab:manual_scores}. 
{\color{red} TODO also say something about which masker is best. LIME was best masker as it resulted in high quality corrections, the baselines didn't work that well. Even with random masker at training and using LIME / Schuster at test time, the generated corrections weren't that great. They're not reported in table 2, but perhaps they should be. } The human evaluation has highest correlation with the SARI metric, displayed in Table~\ref{tab:correlation}. For downstream systems, we will optimize for the SARI metric.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{System} & \textbf{Training}                                              & \textbf{\begin{tabular}[c]{@{}c@{}}Q1\\ Score\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Q2\\ Score\end{tabular}} \\ \midrule
Supervised      & No mutation info                                                  & 2.4                                                         & 2.8                                                         \\
Supervised      & Mutation@source & 2.3                                                         & 2.8                                                         \\
M+C             & LIME mask                                                      & 1.5                                                         & 1.5                                                         \\
Supervised      & Mutation@target & 1.3                                                         & 1.4                                                         \\
M+C             & Schuster mask                                                  & 0.9                                                         & 0.8                                                         \\
M+C             & Diff mask                                                      & 0.4                                                         & 1.3                                                         \\
M+C             & Random mask                                                    & -1.1                                                        & -1.7                                                        \\
Baseline        & Schuster                                                       & -3                                                          & -2.8                                                        \\ \bottomrule
\end{tabular}
\caption{Supervised systems were trained to generate new corrected facts given the evidence using the gold corrections as supervision signal. Additionally, the models were either informed with what mutation was made (mutation@source) or trained to generate the mutation type (mutation@target). The masker+corrector system (M+C) uses a T5 with self-supervision to restore the masked tokens. Maskers were generated with one of the methods described in Section~\ref{sec:method}.}
\label{tab:manual_scores}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}lllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{2}{c}{{\textbf{Q1}}}                                 & \multicolumn{2}{c}{\textbf{Q2}}                                 \\
\multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{\underline{$\mathbf{R_s}$}} & \multicolumn{1}{c}{\textbf{$\mathbf{p}$}} & \multicolumn{1}{c}{\textbf{$\mathbf{R_s}$}} & \multicolumn{1}{c}{\textbf{$\mathbf{p}$}} \\ \midrule
\emph{Human Q2/Q1}                                          & \emph{0.87}                           & $<$\emph{0.001}                           & \emph{0.87}                           & $<$\emph{0.001}                     \\
SARI(Add)                                            & 0.76                           & 0.002                          & 0.79                           & 0.001                          \\
SARI(Del)                                            & 0.73                           & 0.005                          & 0.70                           & 0.007                          \\
SARI(Final)                                          & 0.71                           & 0.006                          & 0.67                           & 0.012                          \\
ROUGE2                                               & 0.60                           & 0.028                          & 0.56                           & 0.044                          \\
ROUGE1                                               & 0.56                           & 0.046                          &        0.51                        &  0.071                              \\
NLI Flips (R-S)                                      & 0.48                           & 0.095                          & 0.53                           & 0.058                          \\
BERTScore                                            & 0.40                           & 0.145                          & 0.50                           & 0.145                          \\
BLEU                                                 & 0.23                           & 0.440                          & 0.32                           & 0.270                          \\ 
\bottomrule
\end{tabular}

\caption{Spearman's Rank Correlation ($R_s$) between manual evaluation (Q1 and Q2) and automated evaluation methods, with reported $p$-value. The "add" component of the SARI score has the highest correlation with human judgements of whether the generated claim is entailed by the evidence.}
\label{tab:correlation}
\end{table}



% Baseline model:
%  - Tal Schuster's fact-guided sentence modification - BLEU score drops from 0.06 to 0.025 with simple swaps and retrained swap model.
%  Sari on original and retrained variants is 30\%  BERTScores 95 for P/R/F1\%. Original is 92.97/94.74/93.84
%  - Baseline model - FEVER classifier trained on 
 
%  Implementation details: 250 LIME examples
 
%\begin{table}[]
%\begin{tabular}{lllll}
%\hline
%Model                 & BLEU  & SARI  & BERTScore & TER   \\ \hline
%Unmodified Hypotheses & 51.96 & 20.99 & 73.11     & 29.33 \\
%Baseline (FEVER)      & 23.14 & 29.31 & 40.78     & 73.50 \\
%%Baseline (LM)         & 17.04 & 29.67 & 0.00      & 75.27 \\
%Schuster              & 31.05 & 42.29 & 51.64     &       \\
%New                   &       &       &           &       \\ \hline
%\end{tabular}
%\end{table}



% \begin{table*}[h]
% \footnotesize
% \begin{tabular}{@{}lccccccc@{}}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{Automated Metrics (\%)}}                                                                           & \multicolumn{3}{c}{\textbf{Human Evaluation (\%)}}                                                                 \\ \cmidrule(l){2-8} 
% \multicolumn{1}{c}{}                                & \textbf{Rouge 1} & \textbf{Rouge 2} & \textbf{Rouge L} & \textbf{\begin{tabular}[c]{@{}c@{}}NLI \\ Label Flips\end{tabular}} & \textbf{Grammatical} & \textbf{Factual}     & \textbf{\begin{tabular}[c]{@{}c@{}}Good \\ Correction\end{tabular}} \\ \midrule
% T5 Supervised (SR) (w/mutation)                         & 79.33            & 69.95            & 77.76            & \multicolumn{1}{l}{}                                                & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                                                \\
% T5 Supervised (SR) (no mutation)                         & 59.14            & 47.89            & 57.98            & \multicolumn{1}{l}{}                                                & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                                                \\
% T5 AutoEncoder (Random)                          &            &         &            &                                                                     &                      &                      &                                                                     \\
% T5 AutoEncoder (String match)                          &            &         &            &                                                                     &                      &                      &                                                                     \\
% T5 AutoEncoder (LIME - Salient Evidence)                          & 60.62            & 41.57            & 60.02            &                                                                     &                      &                      &                                                                     \\
% T5 AutoEncoder (LIME - Full Wiki)                          & 65.40            & 48.62            & 64.88            &                                                                     &                      &                      &                                                                     \\
%                                                     &                  &                  &                  &                                                                     &                      &                      &                                                                     \\ \bottomrule
% \end{tabular}
% \end{table*}


\section{Results}
To do: train system using retrieved evidence too. 

Larger evaluation on top models.



==> 8_conclusions.tex <==
\section{Conclusions}

==> figures/2_construction.tex <==
% \begin{figure*} 
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/fever_construction.pdf}
%     \caption{Construction process of the FEVER dataset which we adapt for Factual Error Correction. For fact verification, systems are trained to perform the role of the blue annotator (finding evidence and using the evidence to label the claim). Our proposal is to use the evidence to not only to find the evidence (blue annotator), but also to use this evidence to undo the mutation introduced by the red annotator.}
%     \label{fig:fever_construction}
% \end{figure*}

\begin{figure} 
    \centering
    \includegraphics[width=\linewidth]{figures/fever_construction_new.pdf}
    \includegraphics[width=\linewidth]{figures/fec_example_claim3.pdf}
    \caption{Contrasting fact verification (FEVER) against error correction. Light gray arrows indicate dataset generation steps. Dark gray arrows indicate system tasks which use Wikipedia evidence to predict claim veracity (for verification) or to make corrections.}
    \label{fig:fever_construction}
\end{figure}

==> figures/3_demo.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/autoencoder.pdf}
    \caption{Training a factual error correction system can be self-supervised by learning to restore masked tokens using the same evidence. At test time, retrieved evidence is used.}
    \label{fig:training}
\end{figure}

==> old/1_intro.tex <==
\section{Introduction}
Fact verification is the task of predicting whether claims are true or false using evidence. With the availability of a number of resources \citep{Wang2017a,Karadzhov2017FullySources,Thorne2018a,Augenstein2019,Wadden2020FactClaims}, the task has attracted significant attention and spawned the development of new models, architectures and approaches. 
With potentially sensitive applications, recent works have focused on building explainable  variants of fact checking \citep{Atanasova2020GeneratingExplanations, Stammbach2020,Kotonya2020}. Exposing the evidence source and decision making process may help the reader uncover subtle issues that cause an automated systems to fail. 
Additionally, using such a data source (or evidence) to continuously update news articles as facts change forms part of vision outlined by \citet{Cohen2011} for automated newsrooms.
Understanding how to make changes to documents based on updated evidence would help fulfill this vision.

%For the FEVER shared task \citep{Thorne2018a}, a large number of systems are a pipeline of information retrieval and classification: relevant evidence is selected from a corpus of texts and used to classify whether the claim is \textsc{Supported} or \textsc{Refuted} by it.

In this paper, we propose \emph{Factual Error Correction}, as an explainable method for performing fact verification. Rather than merely finding evidence or assigning a label, our goal is to rewrite claims so that they are better supported by the retrieved evidence. For example, in Figure~\ref{fig:intro_example}, a claim that would be \textsc{Refuted} by the evidence is rewritten so that it becomes supported by evidence retrieved from Wikipedia.
\input{figures/1_intro_example.tex}
This work extends fact guided sentence modification \citep{Shah2019}
%, which uses masking and self-supervision to obviate the need for additional training data, 
in two ways. Firstly, we incorporate a retrieval component to select evidence for a given claim from a corpus of texts (in our case, Wikipedia). This both demonstrates viability for open-book applications, and represents an advance over previous work in which gold standard evidence is explicitly provided. Furthermore this implicitly regularizes the model to be more selective about which facts are copied from the evidence. %TODO document how the experimental results show this
Secondly, our proposal is to offer a correction regardless of veracity (i.e.\ for  claims supported by evidence, not only refuted). This summarizes the evidence with respect to the claim, helping to resolve half truths, and better informs the end-user of the decision making process, regardless of label.

%While this appears similar to Grammatical Error Correction \citep[GEC]{Knight1994AutomatedDocuments, Ng2014}, with the common goal of providing feedback to an end-user, However, unlike GEC, all our modifications are performed by incorporating external evidence.

%An outline of our proposal is illustrated in Figure~\ref{fig:my_label} 

%This allows highlighting where there is disagreement between the claim and evidence. However, unlike GEC, all our modifications are performed by incorporating external evidence.
%Furthermore, in \emph{factual} error correction, the generated corrections both need to remove the error and be supported by the evidence. 
%Generating corrections provides a mechanism that helps explain the decision making process better than simply assigning a label or highlighting tokens. While generating post-hoc \emph{black-box} model explanations \citep{Ribeiro2016, Ribeiro2018} or interpreting attention \citep{Jain2019,Thorne2019} are informative, they better describe the behaviour of a model -- rather than actionable measures the user can take.
%Corrections inform the end user where the misinformation was introduced, loosely following work on building inherently explainable models (such as \citet{Park2018MultimodalEvidence, Camburu2018}).


{\color{red} TODO Something about the model architecture and our results}



%Rather than modelling the task of fact verification as sentence-labelling (predicting the veracity of a claim as per \citet{Wang2017a}) or , 
%we introduce the task of  (FEC), 
% correcting sentences may allow for updating information written in prose with facts expressed as simple sentences \citep{Shah2019} which would allow for low latency and low cost updates to encyclopedia in reaction to world events.


%,y making meaning-altering rewrites to the claims so that they are better corroborated by available evidence.

This paper presents the following contributions:

\begin{enumerate}
    \item We define the factual error correction task, using %trusted
    evidence retrieved from a knowledge source, such as Wikipedia.%, to update a factually incorrect claim so that it is factually correct
    \item We release a dataset of 90,000 claims, built as an extension to FEVER. All claims are paired with evidence and a either a meaning altering or meaning preserving mutation.
    \item We demonstrate a baseline model trained with self-supervision. This generates corrections that human raters judge as higher quality than an existing model for a related task \citep{Shah2019}.
    \item We evaluate which automated evaluation metrics best correlate with human judgements of whether the error was removed, and whether the corrected sentence is supported by evidence.
\end{enumerate}


\section{Related Work}
A number of recent works offer methods to correct sentences. However, their use of external information differs. The use of external information can be placed on a continuum from no external information at all, to knowledge stored within model parameters, to incorporating external information. We briefly outline key methods and approaches below.

Grammatical Error Correction (GEC) \citep{Knight1994AutomatedDocuments, han-etal-2010-using, Ng2014} is the task of making meaning-\emph{preserving} changes to sentences such that grammatical errors made by language learners are removed. No external knowledge-source is required as the meaning of the sentence is undergoing a surface-level transformation where the (intended) semantic content of the sentence should remain unchanged. 
Recent works model GEC as a sequence-to-sequence task
%han-etal-2010-using
\cite{Yuan2016}, similar to machine translation.
In contrast, the semantic content of sentences undergoing \emph{factual} error correction will be altered, if needed, to better align the meaning to what is presented in the evidence.
It is a requirement that the generated corrections both remove the error from the original claim and be supported by the evidence in the generated correction. 

One potential way to introduce external knowledge when performing error corrections would be to use information stored in the parameters of large-scale pre-trained language models \citep{Petroni2019}. 
In this case, making corrections can be modeled as a variant of cloze-style evaluation \citep{Taylor1953ClozeReadability} -- using the language model to fill in masked tokens.
While such approaches have been employed for
fact verification (for example, \citet{Lee2020LanguageCheckers} used a BERT language model \citep{Devlin2019}), 
these approaches share the following limitations. 
%These may not work well for the following reasons -- 
When masked language models are used to correct claims, the underlying task is to predict the most likely token to replace a mask. Without explicit control \citep{nie-etal-2019-simple}, the most likely token when decoded may not be factually accurate, or supported by the retrieved evidence, commonly referred to as a hallucination \citep{rohrbach-etal-2018-object}.
Furthermore, \emph{even if} the information stored within language model parameters could be reliably expressed as text when making corrections, facts change over time and the need to read information from external evidence becomes greater as the state of the world diverges from the information captured within the model parameters. 
Language models capable of incorporating external information such as RAG \citep{Lewis2020} and REALM \citep{Guu2020}, could be used to incorporate information from Wikipedia, although conditioning generation based on a factual error is an open problem. 
%JT TODO maybe show a better comparison and rewrite this after 



%Language models as knowledge bases \citep{Petroni2019} -- however, rather than using the information stored within the model parameters to generate corrections for the masked tokens, we instead use external evidence.
%is copied from an external knowledge source.


\citet{Shah2019} make meaning-altering updates to sentences in Wikipedia, introducing new ground truth, without the need for additional labeled training data.
Their approach is to mask out salient tokens and train a corrector to replace these from ground truth. In this approach, token salience is predicted by querying a model that is trained to perform fact verification with perturbed inputs. 
Parallels can be drawn between the masker and generating token-level explanations for natural language inference problems where token-level explanations for natural language inference, a related classification task where salient tokens form an explanation. These could be generated generated through perturbing the input, \citep[inter alia]{Ross2017RightExplanations,Li2016,Ribeiro2016}, or by interpreting model weights \citep{} or attention \citep{Jain2019, Thorne2019}. 
While these explanations describe model behaviour, their usage alone can lead to a mismatch between which features are important to the model compared to what features humans would judge as important \citep{Ribeiro2016}.
Generating corrections should provide a mechanism that helps explain the decision making process beyond than simply assigning a label or highlighting salient tokens.
%This allows highlighting where there is disagreement between the claim and evidence. However, unlike GEC, all our modifications are performed by incorporating external evidence.
%Corrections inform the end user where the misinformation was introduced, loosely following work on building inherently explainable models (such as \citet{Park2018MultimodalEvidence, Camburu2018}).



% \citep{Mostafazadeh2016} -- replacing the masked tokens with likely candidates.
%rather than returning explanations to the end user, the explanations are used to mask out tokens.
%Similar shortcomings have been illustrated in sentence-pair classification models, including fact verification \citep{Poliak2018a,Gururangan2018, Schuster2019}.


%\input{figures/2_construction}



%Rather than language modelling, \citet{Shah2019} use an encoder-decoder architecture to introduce updated information into existing Wikipedia sentences. This architecture follows a two-step process, firstly masking salient tokens from the claim and secondly copying-in new tokens from the evidence. 
%As fact-checking is modelled as a sentence pair classification task, similar to Natural Language Inference (NLI), 
%The masking of the salient tokens in this approach is very similar to generating token-level explanations \citep{Thorne2019} -- either through inherent explanation, or through post-hoc explanation using a blackbox interpretation, such as \citep{Ribeiro2016}.
%\citet{Shah2019} use label-changing perturbations to the model input as a signal to fine-tune the attention mechanism, which is thresholded to generate token-level explanations.
%As models become increasingly complex, it becomes more difficult to fully understand and characterize their behaviour. 
%Models capture and exploit the biases present within the training data. 
%By changing the task signature for fact checking from classification to a `correction' generation task, we are training the model to generate its own explanation. 
%Unlike \citet{Camburu2018}, we aim to generate our explanations without the need for supervision using additional training data -- which would have its own biases \citep{Camburu2019}.





==> old/3_task_definition.tex <==
\section{Task Definition}
\label{sec:task}
Factual error correction is the task of making meaning-altering changes to a claim given evidence retrieved from a corpus of documents. %The example illustrated in Figure~\ref{fig:intro_example} demonstrates how the retrieved evidence is retrieved from Wikipedia and integrated into the claim changing the label from refuted to supported.
For a given claim $c$, a factual error correction system must first retrieve evidence $e \in E$ that either \textsc{Supports} or \textsc{Refutes} the claim from a corpus of documents that represent the ground truth where $E \subset \mathcal{E}$. 
To minimize the requirement for additional labeled data, \citet{Shah2019} makes use of a two stage architecture consisting of a \emph{masker} and a \emph{corrector}, outlined below. This enables self-supervision that allows new ground truth facts to be incorporated into sentences on Wikipedia without the need for additional data. 

We build upon this masker-corrector architecture for this paper, however, our definition differs in three ways. Firstly, instead of providing the gold standard ground-truth evidence sentences, we mandate that systems must also first \emph{retrieve} this evidence from a corpus containing ground-truth open-book knowledge. Secondly, instead of assuming that the evidence to be used for claim correction is a single sentence, we allow for multiple sentences retrieved from Wikipedia to be considered.
%using a single simple sentence describing the fact to be introduced to perform the update, 
%we use a set of sentences from Wikipedia to form the evidence. 
Thirdly, we offer a generalization of definition of the masker component, to better align it with existing work on generating token-level explanations.

\paragraph{Retriever}
The first step towards supporting factual error correction is to be able to retrieve evidence from a corpus of documents representing ground-truth knowledge. 
A common model for fact verification is to predict the veracity of a claim $c$, given retrieved set of evidence sentences $E \subset \mathcal{E}$ (in which case the classifier labels whether the claim is \textsc{Supported} or \textsc{Refuted}) or whether there is not enough information to say (in this case the classifier should predict \textsc{NotEnoughInfo}). 
We build upon existing definitions of retrieval for fact verification from FEVER \citep{Thorne2018a}. 
However, rather than use this evidence for labelling the veracity of a claim, we instead use it to form the ground-truth for factual error correction.


\paragraph{Masker}
The input to the masker is a claim $c=(c_1,\ldots,c_n)$ and set of evidence sentences $e \in E$. The masker outputs a masked claim $\tilde{c}$ where for masked tokens $m \in M$, $\tilde{c}_m = \mathtt{\lbrack MASK \rbrack}$. The objective is to generate a set of masks that forms an explanation of which tokens were salient to the classifier, and responsible for the veracity prediction of the claim given evidence. 

Note that this definition differs from that provided by \citet{Shah2019} who use a masking objective to generate $M$ so that for a masked claim $\tilde{c}$ and a single evidence sentence $e_i$ a classifier trained to predict the claim veracity $f(\tilde{c},e_i)$ would predict \textsc{NotEnoughInfo}. Our proposal is a generalization in two ways: firstly, we consider a set of evidence $E$, rather than a single knowledge-book sentence $e_i$ and secondly we remove the dependency for masking to use a classifier to predict a neutral label as we later show two alternative masking objectives which result in higher quality of factual error corrections generated by a downstream system. %that using a the perplexity of a language model objective is sufficient to mask tokens.

\paragraph{Corrector} 
The input to the corrector is a masked sentence $\tilde{c}$ and evidence $E$. The objective is to generate the correction $c'$ such that $E \vDash c'$. The goal of the corrector is to incorporate retrieved evidence $E \subset \mathcal{E}$ into the masked so that
%after FEC, 
the generated correction $c'$ is more strongly supported by this evidence. 

For claims that are refuted by evidence, $E \nvDash c$, the task is to generate a corrected version of the claim $c'$ using the evidence, that both removes the error and becomes supported by the evidence $E\vDash c'$.
For claims that are weakly supported by evidence, $E \vDash c$, as in the case of half-truths or paraphrases, the generated correction should be more strongly supported by the evidence: $E \vDash c' \succcurlyeq E \vDash c$. 



%We first consider methods which do not require additional labeled data based off recent works before presenting language modelling baselines and a fully supervised system highlighting ceiling performance.
%Changes are made to claims regardless of their veracity.




==> old/4_method.tex <==
\section{Method}
\label{sec:method}
The masker-corrector architecture, introduced in Section~\ref{sec:task}, allows for a factual error correction system to be trained without the need for additional labeled data. 
This section first outlines the key components that mask and correct claims, given evidence, We highlight how this architecture enables self-supervision and contrast differences between training and evaluating the system. This section then introduces the retrieval component, and finally discusses fully supervised system that is used to indicate the performance ceiling.


\subsection{Masker}
At test time, the purpose of the masker is to selectively remove tokens that contribute to the factual errors within a claim. 
This broadly follows recent work on generating token-level explanations for the error \citep{Thorne2019a} -- highlighting salient tokens for this label before removing them. 
Once erroneous tokens are masked, new evidence will be introduced from the retriever and by the downstream corrector to restore tokens that have been masked out.

During training, however, the masker serves a different purpose. The masker is used to generate a supervision signal for the downstream corrector module, indicated in Figure~\ref{fig:training}.
Before training, tokens are removed from the claim by the masker, generating $\tilde{c}$. 
Rather than generating a correction with new ground-truth, the training objective of the downstream corrector module is to recover the original meaning, using the external evidence such that $correct(\tilde{c},E) = c' = c$.
The masker used at test time doesn't necessarily have to be the same as the masker used to train the corrector.  

We study how the choice of masker at training and test time influences the quality of corrections generated by the FEC system. There is a trade-off between the time taken to generate the masks, and how the masked tokens agree with human judgements of token importance \citep{Thorne2019}. On one extreme, tokens could be randomly masked, following a similar training strategy to BERT \citep{Devlin2019} or the T5 \citep{Raffel2020} pre-trained language models. Generating large quantities of training data is possible without having to query an oracle model. On the other extreme, one could perturb the input to an oracle fact verification model that is trained to predict the veracity of a claim given evidence. Querying this model with perturbed inputs using a black-box model explanation technique such as LIME \citep{Ribeiro2016} agrees more strongly with human judgements of important tokens but requires a number of queries to the oracle model to generate the token-level explanation.

In previous work, \citet{Shah2019} use white-box model explanations to mask the input prior to correction using attention as an explanation mechanism. This requires a single query to an ESIM model \citep{Chen2016} that is trained to predict veracity of a claim given evidence. However attention alone is insufficient to generate quality explanations \citep{Jain2019}. To overcome this limitation, the authors fine-tune the attention mechanism with hand-crafted constraints to better align the generated masks with the saliency of tokens. 

We experiment with 3 variants of the masker (and 2 baselines) used to generate the training and test data for the downstream correction module as follows: 

\input{figures/3_demo}

\begin{description}
    \item[Black-box masker] Tokens are masked from the claim using predictions from a sentence pair classification model trained on instances from the FEVER dataset. This model is a fine-tuned BERT classifer that is representative of the state of the art for the FEVER shared task \citep{Thorne2018b}. We use LIME \cite{Ribeiro2016} to generate explanations of which tokens from the claim are salient to a sentence pair classifier trained on claims and evidence. This method perturbs instances by masking tokens and uses the change in labels to train a linear classifier that weights the importance of each token.
    
    \item[White-box masker] We use the masker from \citet{Shah2019} which is an ESIM \citep{Chen2016} sentence pair classifier. Token-level explanations are generated through thresholding attention values. %Unlike \citet{Thorne2019a}, there is additional supervision: instances are perturbed by masking tokens. 
    Tokens are masked that cause a change from a either the \textsc{Supports} or \textsc{Refutes} labels to \textsc{NotEnoughInfo}. 
    After the classifier is trained, it undergoes a second-round of fine-tuning where the model is penalized for attending to tokens which, when removed, do not change the label from \textsc{Supports} or \textsc{Refutes} to \textsc{NotEnoughInfo} an additional loss function, controlled by a hyper-parameter also penalizes the model for masking too-many or too-few tokens.
    

    \item[Language model masker] We evaluate whether it's possible to generate meaningful masks without the need for a model trained to perform fact verification. We use a BERT pre-trained language model \citep{Devlin2019} to measure the surprisal of tokens in the claim. 
    As we wish to identify tokens which introduce misinformation in the claim, our hypothesis is that a language model captures world knowledge \cite{Petroni2019} and that tokens contrary to this knowledge may have a higher surprisal. This language model has no additional task-specific fine-tuning.
    
    \item[Baselines] We additionally consider two two simple baseline maskers: randomly masking a subset of tokens and also masking tokens which are not in common between the claim and the evidence.
\end{description}

\subsection{Corrector}
The corrector model is responsible for replacing masked tokens with new tokens conditioned on the retrieved evidence. The input is the masked claim, $\tilde{c}$ and evidence E. The generated output, $c'$, is required to be supported by the evidence $E \vDash c'$.

In previous work, \citet{Shah2019} use a dual-encoder pointer generator network \citep{See2017GetNetworks} to independently encode a single evidence sentence and the masked claim using LSTMs \citep{Hochreiter1997}. This pointer network uses that trained to recover masked tokens through self-supervision. During training, the corrector is trained to recover the masked tokens using the evidence -- illustrated in Figure~\ref{fig:training}. At test time, different evidence is used (for example, retrieved evidence that \textsc{Refutes} a claim), the hypothesis is that conditioning on this different evidence would cause the tokens replacing the masked tokens to be supported by the new evidence -- correcting any factual errors

We propose an alternative approach using an encoder-decoder transformer model instead of a pointer generator network. 
We experiment with using T5 transformer \citep{Raffel2020}, pretrained with a sequence to sequence masked language modelling objective.
This pretraining objective is very similar to the task of correction, although there is no conditioning on evidence.
To condition on evidence, we additionally fine-tuning the T5 transformer with the same objective as the pointer generator network. 
Although, rather than independently encoding the evidence and claim, we jointly encode them by concatenating the two. 
This would allow the self-attention layers within the transformer to better capture long-range dependencies between the evidence and the claim \citep{Vaswani2017}.
%The model is trained for up to 8 epochs, the weights from the model which has the highest Rouge2 score on the validation set is retained for evaluation.
%Each masked token is replaced with a unique, and ordered masking token {\tt <extra\_id\_i>} where $i$ corresponds to the index of the masked token (out of all masked tokens).
We evaluate the quality of corrections trained using different maskers, described in Section~\ref{sec:method:masker}, as this is likely to impact the effectiveness of the generated correction.

To evaluate the impact of conditioning on evidence, we consider an unconditioned language model, replicating the Language Models as Knowledge Bases hypothesis introduced by \citet{Petroni2019}. This would consider correcting claims using the implicit knowledge stored within the model parameters rather than using external evidence.

\subsection{Retriever}
The retriever must return evidence, in the form of sentences, from a corpus of documents that form the ground-truth for masking and correcting the claims. In our case the ground-truth comes from a static snapshot of Wikipedia.  For a given claim $c$, the retriever must select a minimal subset of claims $E\subset\mathcal{E}$ that would be sufficient to predict the veracity of the claim with a classifier: $f(c,E)\in \{Supports,Refutes\}$.

Information retrieval for fact verification is an active area of research. For our initial study on error correction, we consider three approaches existing that are representative of the state of the art for the task. We compare retrieval with TF-IDF \citep{Chen2017}, Generative Retrieval \citep{DeCao2020}, and inner product search between encoded representations with DPR \citep{Karpukhin2020}. Each method is formally described in Section~\ref{sec:experiment}.


\subsection{Full Supervision}
With full supervision of source claim, evidence and target corrections, factual error correction may be modelled as a sequence-to-sequence language generation task over the claim directly, without the need for masking. 
For this model, the input is the source claim and evidence, concatenated together, and the output is the target correction. 
The dataset we introduce in Section~\ref{sec:data} contains paired source and target claims which can be used to supervise training.
We use this data to estimate the ceiling performance of a factual error correction system (assuming sufficient training data is available) that other methods can be compared against.
In this paper, we use an auto-regressive encoder-decoder transformer model, T5 \citep{Raffel2020}, which we fine-tune on the FEC dataset.


% \paragraph{Mutation type supervision:} We additionally evaluate use of the mutation type metadata as an additional supervision signal: (1) the impact of knowing the mutation type in advance could condition the model to generate a different output if provided as an input, and (2) jointly predicting the mutation type when generating the target correction may improve the quality of generated correction and provide useful for downstream applications.

% \paragraph{Evidence source:} The noise introduced by inaccurate evidence may impact the quality of generated explanations. We evaluate 3 sources of evidence in this baseline: (1) the original sentence used to generate the claim: this should contain the facts which were summarized when generating the target correction (2) the evidence selected by annotators from Wikipedia: this may be noisier than the original sentences, but as annotators have labelled these additional sentences as sufficient to support or refute the claim, they are likely to contain enough information that would enable factual error correction. (3) We finally evaluate using evidence returned from information retrieval model, as we cannot expect perfect evidence to be returned when applying the model in a real-world setting. % we must evaluate the model's ability to generate corrections in a noisy environment.
 
 
% \subsection{Baselines}

% The contribution we present in this paper uses a sequence-to-sequence model trained as an auto-encoder to recover missing tokens from a source sentence containing evidence. At training time, we selectively mask tokens from true claims, supported by evidence and use a language model to recover the missing tokens from the Wikipedia evidence. 





% \subsection{Fact-guided sentence modification baseline}
% We adapt and evaluate fact-guided sentence modification \cite{Shah2019} as a baseline. This is a two-step approach to sentence modification: (1) masking salient tokens that are influential for a sentence classification task and (2) copying tokens from a reference sentence to replace the masked tokens with updated facts. 
% The original application of this work is to substitute information from factoid sentences to update information into Wikipedia. We re-train this model using the code available from the authors\footnote{\url{https://github.com/TalSchuster/TokenMasker}} to perform the task of factual error correction, inputting a claim and evidence sentence from Wikipedia, and generating the correction for the claim.

% This baseline model does not require supervision for the factual error correction part of the task and relies only on the supervision from a sentence-pair classification task. We use this model to recover a corrected claim without direct supervision, using canonical evidence from the original Wikipedia sentence.  Implementation details are as follows:

% \paragraph{Masker: } The model is trained as a sentence-pair classifier on the original FEVER dataset, predicting whether a claim is supported, refuted from a Wikipedia sentence or whether the is not enough information. The model is based on the AllenNLP implementation \citep{Gardner2017} of an a ESIM \cite{Chen2019} model. Thresholded attention weights are used to mask salient tokens, this is trained with an objective whereby masking these tokens would result in a polar classification of a sentence pair (supports/refutes) changing the label to not enough info with a regularization term controlling the proportion of masked tokens.

% \paragraph{Copy mechanism: } A second pointer-generator model, is independently trained to input a pair of sentences, one with masks and a reference sentence, and is distantly trained to recover the information deleted through the masking process through copying tokens from the reference sentence through ensuring agreement with a natural language classifier.


% \subsection{Dual masker baseline}
% Without an additional model, we evaluate masking both the claim and evidence sentences used in a sentence-pair classification model trained on the FEVER dataset. Salient tokens from both the claim and evidence are masked using LIME as this has been found to generate more consistent explanations for sentence-pair classification tasks than attention based masking: \cite{Thorne2019a}. We experiment with two model-configurations: (1) naive substitution of masked tokens using largest contiguous span, and, (2) using back-translation to summarize key facts (e.g. like in SEARs)



==> old/5_data.tex <==
\section{Data}
\label{sec:data}

\input{figures/2_construction}


To train the systems that use the masker-corrector architecture, we require claims, accompanied with evidence. 
We make use of a FEVER \citep{Thorne2018a}, a common fact verification dataset as the basis for experiments for factual error correction. 
FEVER contains 185k instances which are annotated with corresponding evidence from Wikipedia and a label as to whether the claim is \textsc{Supported} or \textsc{Refuted} by it.  

To comprehensively evaluate the corrections generated by FEC systems, manual evaluation is required. However, this comes with a high cost and is not suitable for system debugging and development. To support automated evaluation, we make use of intermediate data from FEVER to generate reference sentences for corrections. 
%Explicitly say we could have used otehr data with gold standard evidence and data. Further annotations help us evaluate the corrections. 
%The FEVER dataset \cite{Thorne2018a} contains 185k claims accompanied by evidence and a
%label indicating whether a claim was \textsc{Supported} or \textsc{Refuted} by the evidence. For one third of the claims, evidence in Wikipedia could not be found by annotators. These claims are labelled as \textsc{NotEnoughInfo} (abbreviated NEI).
The claims in FEVER were generated by annotators in a two-stage process. Annotators both extracted facts from Wikipedia and then performed meaning altering perturbations called \emph{mutations} over these extracted facts, illustrated Figure~\ref{fig:fever_construction}. 
Our reference corrections are \emph{undoing} the mutations introduced by the annotators, restoring the original extracted facts.
%First, information was extracted from randomly sampled Wikipedia sentences as short factoid statements (referred to as extracted facts). Following this, the sentences are \emph{mutated} by the same annotator who extracted the facts by performing one of the
%Under agreement with the FEVER task organizers, we incorporate these annotations into the FEC dataset which we release with this paper.

%In a separate annotation process, different annotators use Wikipedia to find evidence and label whether the claim is \textsc{Supported} or \textsc{Refuted} by this evidence, or, label whether there is not enough information.
%The FEVER shared task challenges systems to perform the role of the second annotation process (indicated with the blue person in Figure~\ref{fig:fever_construction}). In the official dataset release, claims are accompanied with the evidence to support or refute them and the veracity label. It does not contain the intermediate annotation artefacts, such as the extracted facts and Wikipedia sentences, which described how the claims were generated from Wikipedia documents. 
%In this paper, we make use of these intermediate data, having obtained these from the task organizers. These annotations will be used to construct a benchmark dataset for factual error correction, which will be released with this paper. 

The FEC dataset we release in this paper is constructed from adapting FEVER. In the dataset construction for FEVER, human annotators extracted facts from Wikipedia sentences. Facts, $f$, undergo mutation by the same human annotator, performing potentially meaning-altering rewrite operations, $o$, to generate claims $c=mutate(f,o)$.

The veracity of claims is now unknown and must be verified through retrieving a set of evidence sentences $E\subset\mathcal{E}$ from Wikipedia. For the veracity prediction task in FEVER, this evidence is used to label whether the claim is \textsc{Supported} or \textsc{Refuted} by the evidence. For error correction, this evidence is instead used to condition the generation of the corrected claim $c'$. Extracted facts $f$ were not released in the FEVER dataset. For automated evaluation, we consider the extracted fact, $f$ as a reference sentence for the corrected claim $c'$. While this reference sentence isn't needed for training a masker-corrector system, we release the annotations to both support automated system evaluation, and to train a baseline system with full supervision for comparison.

% \subsection{Dataset Construction}
% The following section describes in detail the dataset collection process from FEVER and a mapping used to construct a dataset for the factual error correction task.

% \paragraph{1) Original Wikipedia sentence:} during construction of FEVER, a sentence sampled the introduction sections of the most-popular 50,000 Wikipedia pages was presented to annotators. This sentence can be used in FEC as \emph{canonical evidence} that is highly trusted and can be used to recover the original factual meaning of claims.

% \paragraph{2) Extracted Wikipedia fact:} using the original Wikipedia sentence, FEVER annotators were asked to summarize it into short facts. These form \emph{target corrections} used to evaluate factual error correction systems and for supervised training. These target corrections represent ground truth that can be evidenced by the canonical evidence in the original Wikipedia sentence.

% \paragraph{3) Mutated Wikipedia facts (claims):} Wikipedia facts were mutated into claims by FEVER annotators through both meaning-preserving and meaning-altering creative rewrites. Without evidence, we may not know whether these claims are true or false. In this paper, these form the \emph{source claims} which are of unknown veracity and require factual error correction. There is additional optional supervision in the form on the \emph{mutation type} metadata. We evaluate its effect and whether it is required for the error correction task through experimentation, reported in Section~\ref{sec:evaluation}.

% \paragraph{4) Evidence for claims:} Annotators were asked to find evidence that supports (would provide an inference that indicates the claim is true) or refutes (would provide an inference that indicates the claim is false) the claim. Evidence is provided as a set of sentences, referencing spans extracted from a pre-processed snapshot of Wikipedia.  For the factual error correction task, we consider this as a more noisy source of information for correction (in comparison to 1), we additionally evaluate an end-to-end pipeline task, using evidence retrieved using an information retrieval component.

% % TODO move to "Experiments"
% \subsection{Dataset Statistics}
% We retain the training, dev and test splits of the FEVER dataset released by \citet{Thorne2018a} where the entities are disjoint between the different dataset partitions.
% Our dataset release is a subset of the FEVER dataset, as the claims in FEVER were a mixture of original and mutated claims whereas our dataset release is a surjective mapping from mutated claims to original claims.

\begin{table}[h]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Label}}} & \multicolumn{3}{c}{\textbf{Instance Count}}                                     \\ \cline{2-4} 
\multicolumn{1}{c}{}                                & \textbf{Train}            & \textbf{Dev}             & \textbf{Test}            \\ \midrule
Supports                                            & 37961                     & 1477                     & 1593                     \\
Refutes                                             & 20075                     & 2091                     & 2289                     \\
Not Enough Info                                     & 21934                     & 1870                     & 2037                     \\ \midrule
All classes                                         & \multicolumn{1}{l}{79970} & \multicolumn{1}{l}{5438} & \multicolumn{1}{l}{5919} \\
\bottomrule
\end{tabular}
\caption{Instance counts by class for training, development and test dataset partitions}

\end{table}




To train the systems that use the masker-corrector architecture, we require claims, accompanied with evidence. 
We make use of a FEVER \citep{Thorne2018a}, a common fact verification dataset as the basis for experiments for factual error correction. 
FEVER contains 185k instances which are annotated with corresponding evidence from Wikipedia and a label as to whether the claim is \textsc{Supported} or \textsc{Refuted} by it.  

To comprehensively evaluate the corrections generated by FEC systems, manual evaluation is required. However, this comes with a high cost and is not suitable for system debugging and development. To support automated evaluation, we make use of intermediate data from FEVER to generate reference sentences for corrections. 
%Explicitly say we could have used otehr data with gold standard evidence and data. Further annotations help us evaluate the corrections. 
%The FEVER dataset \cite{Thorne2018a} contains 185k claims accompanied by evidence and a
%label indicating whether a claim was \textsc{Supported} or \textsc{Refuted} by the evidence. For one third of the claims, evidence in Wikipedia could not be found by annotators. These claims are labelled as \textsc{NotEnoughInfo} (abbreviated NEI).
The claims in FEVER were generated by annotators in a two-stage process. Annotators both extracted facts from Wikipedia and then performed meaning altering perturbations called \emph{mutations} over these extracted facts, illustrated Figure~\ref{fig:fever_construction}. 
Our reference corrections are \emph{undoing} the mutations introduced by the annotators, restoring the original extracted facts.
%First, information was extracted from randomly sampled Wikipedia sentences as short factoid statements (referred to as extracted facts). Following this, the sentences are \emph{mutated} by the same annotator who extracted the facts by performing one of the
%Under agreement with the FEVER task organizers, we incorporate these annotations into the FEC dataset which we release with this paper.

%In a separate annotation process, different annotators use Wikipedia to find evidence and label whether the claim is \textsc{Supported} or \textsc{Refuted} by this evidence, or, label whether there is not enough information.
%The FEVER shared task challenges systems to perform the role of the second annotation process (indicated with the blue person in Figure~\ref{fig:fever_construction}). In the official dataset release, claims are accompanied with the evidence to support or refute them and the veracity label. It does not contain the intermediate annotation artefacts, such as the extracted facts and Wikipedia sentences, which described how the claims were generated from Wikipedia documents. 
%In this paper, we make use of these intermediate data, having obtained these from the task organizers. These annotations will be used to construct a benchmark dataset for factual error correction, which will be released with this paper. 

The FEC dataset we release in this paper is constructed from adapting FEVER. In the dataset construction for FEVER, human annotators extracted facts from Wikipedia sentences. Facts, $f$, undergo mutation by the same human annotator, performing potentially meaning-altering rewrite operations, $o$, to generate claims $c=mutate(f,o)$.

The veracity of claims is now unknown and must be verified through retrieving a set of evidence sentences $E\subset\mathcal{E}$ from Wikipedia. For the veracity prediction task in FEVER, this evidence is used to label whether the claim is \textsc{Supported} or \textsc{Refuted} by the evidence. For error correction, this evidence is instead used to condition the generation of the corrected claim $c'$. Extracted facts $f$ were not released in the FEVER dataset. For automated evaluation, we consider the extracted fact, $f$ as a reference sentence for the corrected claim $c'$. While this reference sentence isn't needed for training a masker-corrector system, we release the annotations to both support automated system evaluation, and to train a baseline system with full supervision for comparison.

% \subsection{Dataset Construction}
% The following section describes in detail the dataset collection process from FEVER and a mapping used to construct a dataset for the factual error correction task.

% \paragraph{1) Original Wikipedia sentence:} during construction of FEVER, a sentence sampled the introduction sections of the most-popular 50,000 Wikipedia pages was presented to annotators. This sentence can be used in FEC as \emph{canonical evidence} that is highly trusted and can be used to recover the original factual meaning of claims.

% \paragraph{2) Extracted Wikipedia fact:} using the original Wikipedia sentence, FEVER annotators were asked to summarize it into short facts. These form \emph{target corrections} used to evaluate factual error correction systems and for supervised training. These target corrections represent ground truth that can be evidenced by the canonical evidence in the original Wikipedia sentence.

% \paragraph{3) Mutated Wikipedia facts (claims):} Wikipedia facts were mutated into claims by FEVER annotators through both meaning-preserving and meaning-altering creative rewrites. Without evidence, we may not know whether these claims are true or false. In this paper, these form the \emph{source claims} which are of unknown veracity and require factual error correction. There is additional optional supervision in the form on the \emph{mutation type} metadata. We evaluate its effect and whether it is required for the error correction task through experimentation, reported in Section~\ref{sec:evaluation}.

% \paragraph{4) Evidence for claims:} Annotators were asked to find evidence that supports (would provide an inference that indicates the claim is true) or refutes (would provide an inference that indicates the claim is false) the claim. Evidence is provided as a set of sentences, referencing spans extracted from a pre-processed snapshot of Wikipedia.  For the factual error correction task, we consider this as a more noisy source of information for correction (in comparison to 1), we additionally evaluate an end-to-end pipeline task, using evidence retrieved using an information retrieval component.

% % TODO move to "Experiments"
% \subsection{Dataset Statistics}
% We retain the training, dev and test splits of the FEVER dataset released by \citet{Thorne2018a} where the entities are disjoint between the different dataset partitions.
% Our dataset release is a subset of the FEVER dataset, as the claims in FEVER were a mixture of original and mutated claims whereas our dataset release is a surjective mapping from mutated claims to original claims.

\begin{table}[h]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Label}}} & \multicolumn{3}{c}{\textbf{Instance Count}}                                     \\ \cline{2-4} 
\multicolumn{1}{c}{}                                & \textbf{Train}            & \textbf{Dev}             & \textbf{Test}            \\ \midrule
Supports                                            & 37961                     & 1477                     & 1593                     \\
Refutes                                             & 20075                     & 2091                     & 2289                     \\
Not Enough Info                                     & 21934                     & 1870                     & 2037                     \\ \midrule
All classes                                         & \multicolumn{1}{l}{79970} & \multicolumn{1}{l}{5438} & \multicolumn{1}{l}{5919} \\
\bottomrule
\end{tabular}
\caption{Instance counts by class for training, development and test dataset partitions}

\end{table}


==> old/6_evaluation.tex <==
\section{Evaluation Metrics}
Corrections generated by a factual error correction system must be intelligible, be supported by evidence, and remove the error from the claim. We evaluate system output with double-blind human evaluation, asking the following 3 questions, pertaining to 3 requirements. 

\paragraph{Q1 - Intelligibility} Annotators are shown the correction and asked: ``is the correction an intelligible fact?'' and must give a binary answer. For corrections that are nonsense or do not form an intelligible fact, are given a negative rating.

\paragraph{Q2 - Supported by Evidence} Annotators are shown the correction and the evidence and asked a binary question ``is the correction supported by the evidence?'' We use definition of Supported from the FEVER task \citep{Thorne2018a}.

\paragraph{Q3 - Error correction} Annotators are shown the claim, evidence and the correction and asked ``did the system correct the error in the input, accordign to the evidence?''. The annotation is 3 way: (1) nothing useful; (2) error removed, but not corrected; (3) corrected.
%highlight the differnece to Shah

% 3 requirements
% Q1 Intelligible?
% +1 Intelligible 
% 0 Not intelligible

% (IF Q1=+1) Q2 was output supported by the evidence? - No reference to input
% +1 Supported 
% 0 Not supported (or refuted) by evidence


% (IF Q2=+1) Q3 did output correct the error in the input, according to the evidence?
% +2 Corrected 
% +1 Removed, but not corrected 
% 0 Nothing useful
% This is a novel Q compared to schuster - mention in task definition
% pertinent because we use multi-sentence evidence (especially from retriever) where simply copying one of these sentences would not be sufficient to correct the error


% \paragraph{Requirement 1} Is the newly generated claim supported by the evidence? %(5 answers).
% Possible answers: \textsc{Supported} (the generated claim is fully supported by evidence), \textsc{Half-Supported} (the generated claim is supported, but unrelated to the original), \textsc{Not Enough Info} (given the evidence, we cannot say whether the claim is supported or refuted), \textsc{Refuted} (given the evidence, one would assume the claim is false), \textsc{Unintelligible} (the system output was not an intelligible English sentence). 

% \paragraph{Requirement 2} Does the corrected claim address the error that was present in the input claim? 
% \textsc{Yes} (the error was removed), \textsc{Half-right} (error removed, but the newly generated claim not supported by evidence), \textsc{Neutral} (The error was removed but the corrector made a mistake when generating the new claim), \textsc{No} (the error was not removed), \textsc{Unintelligable}.

% The systems were scored on a scale with +3 and +2 for being perfectly right, 0 for neutral/nei and -2 for unchanged/refuted and -3 for unintelligable. 

% 2 requirements 
% Q1 was output supported by the evidence?
% Q2 did output correct the error in the input, according to the evidence?
%Factual error correction systems must use evidence to remove 

\medskip\noindent
Human evaluation of the generated outputs is time consuming and does not scale. Additionally, disagreements between annotators may make evaluation more challenging. 
To estimate system performance for development, we consider automated evaluation.
This considering the similarity of the correction $c'$ to a reference sentence. 
Automated metrics, such as \textsc{Bleu} \citep{Papineni2002} and \textsc{Rouge} \citep{Lin2004} consider the number of 
token units 
n-grams
in common -- evaluating precision and recall respectively. 
The SARI \cite{Xu2016OptimizingSimplification} document simplification metric provides additional insight which can be used to measure factual error correction -- the summarizing metric considers deleted tokens from the original sentence as part of the evaluation, as well as how many added tokens are in common with the reference.
An issue with these automated metrics is that they consider the proportion of tokens in common with the reference. Perturbations, such as the presence of a token that negates the meaning, are not proportionally scored by their impact on the sentence-level semantics.

Another evaluation method we can consider is to use a classifier to predict whether the newly generated correction is \textsc{Supported} by the evidence. A successful factual error correction system, given a claim refuted by evidence as input, 
would make corrections such that the predicted label flips to supported. Sentence-pair classifiers like this have high accuracy of the FEVER dataset -- with an accuracy of over 90\% -- %however, this error rate 
nevertheless they
may introduce additional noise in the scoring. Furthermore, as the corrected claims are likely 
%to be outside of the distribution of
to differ from the
claims in the original dataset, the accuracy of this evaluation metric might be further reduced.
%this measure of success may be less reliable on this task.

% We consider manual evaluation, which has the benefit of using human judgements to predict whether the generated sentences are supported given the available evidence and \emph{correct} the errors present in the original sentences. However, this evaluation metric has a cost associated with it as well as the potential to introduce noise through disagreements on human judgements. 

To indicate which automated measures best align with human judgements, we compute Spearman's correlation between the automated metrics and human judgments in a pilot study evaluation. To convert the answers to the questions to a score, we assign $0$ for a negative answer and $1$ for a positive answer. For Q3 which has a 3-way annotation, the `half-right' choice is awarded half a point.
In system design, we optimize the systems for metrics which have high correlation with human judgement and low $p$-value.


